Joint Learning of Linear Time-Invariant Dynamical Systems

Linear time-invariant systems are very popular models in system theory and applications. A fundamental problem in system identification that remains rather unaddressed in extant literature is to leverage commonalities amongst related linear systems to estimate their transition matrices more accurately. To address this problem, the current paper investigates methods for jointly estimating the transition matrices of multiple systems. It is assumed that the transition matrices are unknown linear functions of some unknown shared basis matrices. We establish finite-time estimation error rates that fully reflect the roles of trajectory lengths, dimension, and number of systems under consideration. The presented results are fairly general and show the significant gains that can be achieved by pooling data across systems in comparison to learning each system individually. Further, they are shown to be robust against model misspecifications. To obtain the results, we develop novel techniques that are of interest for addressing similar joint-learning problems. They include tightly bounding estimation errors in terms of the eigen-structures of transition matrices, establishing sharp high probability bounds for singular values of dependent random matrices, and capturing effects of misspecified transition matrices as the systems evolve over time.

==> pkg_macros.tex <==
\usepackage[colorlinks=true, linkcolor=blue, citecolor=blue]{hyperref}       % hyperlinks
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{color}
\usepackage{xcolor}
% \usepackage{microtype}      % microtypography
\usepackage{amsmath, amsthm}
\usepackage{amssymb, amsfonts, mathtools, enumitem, amsbsy}
\usepackage{graphicx}
% \usepackage{algorithm}
\usepackage{pifont}
% \usepackage{subcaption}
\usepackage{float}
\usepackage{subfigure}
% If you use natbib package, activate the following three lines:
\usepackage[round]{natbib}
\renewcommand{\bibname}{References}
\renewcommand{\bibsection}{\subsubsection*{\bibname}}
\usepackage{wrapfig}
% If you use BibTeX in apalike style, activate the following line:
\bibliographystyle{plainnat}

\newcommand{\R}{\mathbb{R}}
\newcommand{\wtilde}[1]{\widetilde{#1}}
\newcommand{\wbar}[1]{\overline{#1}}
\newcommand{\what}[1]{\widehat{#1}}
\newcommand{\dn}{\mathop{\mathrm{dn}}}
\newcommand{\up}{\mathop{\mathrm{up}}}

\newtheorem*{theorem*}{Theorem}
\newtheorem*{lemma*}{Lemma}
\newtheorem*{corollary*}{Corollary}
\newtheorem*{proposition*}{Proposition}
% \newtheorem*{thm*}{Theorem}
% \newtheorem*{lem*}{Lemma}
% \newtheorem*{cor*}{Corollary}
% \newtheorem*{prop*}{Proposition}

% Latex macros for notation borrowed from Kazem's papers
\newcommand{\Mnorm}[1]{{\left\vert\kern-0.30ex\left\vert\kern-0.30ex\left\vert #1 
		\right\vert\kern-0.30ex\right\vert\kern-0.30ex\right\vert}}
\newcommand{\eigmax}[1]{\left|\lambda_{\max}\left( #1 \right)\right|}
\newcommand{\eigmin}[1]{\left|\lambda_{\min}\left( #1 \right)\right|}

\newcount\Comments  % 0 suppresses notes to selves in text
\Comments=1% TODO: change to 0 for final version
\definecolor{darkred}{rgb}{0.7,0,0}
\definecolor{drkgreen}{rgb}{0,0.5,0}
\definecolor{purple}{rgb}{0.6,0.0,0.8}
\newcommand{\kibitz}[2]{\ifnum\Comments=1{\textcolor{#1}{\textsf{\footnotesize #2}}}\fi}
\newcommand{\ambuj}[1]{\kibitz{purple}{[AT: #1]}}
\newcommand{\aditya}[1]{\kibitz{drkgreen}{[AM: #1]}}
\newcommand{\george}[1]{\kibitz{magenta}{[GM: #1]}}
\newcommand{\kazem}[1]{\kibitz{red}{[MF: #1]}}

==> title_abstract.tex <==
\twocolumn[
\icmltitle{Joint Learning of Linear Time-Invariant Dynamical Systems}

% It is OKAY to include author information, even for blind
% submissions: the style file will automatically remove it for you
% unless you've provided the [accepted] option to the icml2022
% package.

% List of affiliations: The first argument should be a (short)
% identifier you will use later to specify author affiliations
% Academic affiliations should list Department, University, City, Region, Country
% Industry affiliations should list Company, City, Region, Country

% You can specify symbols, otherwise they are numbered in order.
% Ideally, you should not use this facility. Affiliations will be numbered
% in order of appearance and this is the preferred way.
\icmlsetsymbol{equal}{*}

\begin{icmlauthorlist}
\icmlauthor{Aditya Modi}{ms}
\icmlauthor{Mohamad Kazem Shirani Faradonbeh}{uga}
\icmlauthor{Ambuj Tewari}{um}
\icmlauthor{George Michailidis}{ufl}
\end{icmlauthorlist}

\icmlaffiliation{ms}{Microsoft, Mountain View}
\icmlaffiliation{um}{Department of Statistics, University of Michigan Ann Arbor}
\icmlaffiliation{uga}{Department of Statistics, University of Georgia}
\icmlaffiliation{ufl}{Department of Statistics, University of Florida}

\icmlcorrespondingauthor{Aditya Modi}{admodi@umich.edu}
\icmlcorrespondingauthor{Mohamad Kazem Shirani Faradonbeh}{mohamadksf@uga.edu}

% You may provide any keywords that you
% find helpful for describing your paper; these are used to populate
% the "keywords" metadata in the PDF but will not be shown in the document
\icmlkeywords{}

\vskip 0.3in
]

% this must go after the closing bracket ] following \twocolumn[ ...

% This command actually creates the footnote in the first column
% listing the affiliations and the copyright notice.
% The command takes one argument, which is text to display at the start of the footnote.
% The \icmlEqualContribution command is standard text for equal contribution.
% Remove it (just {}) if you do not need this facility.

\printAffiliationsAndNotice{}  % leave blank if no need to mention equal contribution
% \printAffiliationsAndNotice{\icmlEqualContribution} % otherwise use the standard text.

\begin{abstract}
Stochastic linear time-invariant dynamical systems are among the most popular models in various areas of system theory and applications. 
A fundamental problem that remains unaddressed is that of utilizing commonalities of related systems to improve the estimation of transition matrices. 
To address that, this work initiates study of reliable methods for jointly learning multiple systems that their transition matrices are \emph{uncertain} linear functions of \emph{uncertain} shared bases. 
We establish finite-time error rates that fully present the roles of \emph{trajectory lengths}, \emph{dimension}, and \emph{number of systems}. 
The presented results are fairly general, indicate the significant gains of pooling data across systems in comparison to individual learning, and are shown to be \emph{robust} against model misspecifications. 
To obtain the results, we develop novel techniques that are of broader interest in similar joint-learning settings. 
The technical novelties include establishing tight learning rates with respect to the eigen-structure of transition matrices and unknown deviations from the model, as well as spectral analysis of dependent random matrices.
\end{abstract}
